A Family of Pretrained Transformer Language Models for Russian

Transformer language models (LMs) are fundamental to NLP research methodologies and applications in various languages. However, developing such models specifically for the Russian language has received little attention. This paper introduces a collection of 13 Russian Transformer LMs, which spans encoder (ruBERT, ruRoBERTa, ruELECTRA), decoder (ruGPT-3), and encoder-decoder (ruT5, FRED-T5) architectures. We provide a report on the model architecture design and pretraining, and the results of evaluating their generalization abilities on Russian language understanding and generation datasets and benchmarks. By pretraining and releasing these specialized Transformer LMs, we aim to broaden the scope of the NLP research directions and enable the development of industrial solutions for the Russian language.

==> tables/parameters.tex <==

\begin{table*}[]
\scriptsize
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{ccc}
\toprule

 

\textbf{Task}           & \textbf{Tuning parameters} & \textbf{Generation parameters} \\ \midrule 
Detoxification &      &                                \\ 
Simplification &       num\_train\_epochs=10, learning\_rate = 1e-5                       &                             top\_p=0.8,     repetition\_penalty=1.5                                                \\ 
Summarization &            &  \\ 

\bottomrule
\end{tabular}
\caption{Hyperparameter configurations for Natural Language Generation tasks.}\label{tab:parameters}
\end{table*}

==> tables/rucola.tex <==
\begin{table}[t!]
\centering
    \tiny 
    \resizebox{\columnwidth}{!}{\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model} & \textbf{Acc.} & \textbf{MCC} \\ \midrule

%\multicolumn{2}{c}{\textbf{Overall}} & \multicolumn{2}{c}{\textbf{In-domain}} & \multicolumn{2}{c}{\textbf{Out-of-domain}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
% & \textbf{Acc.} & \textbf{MCC} & \textbf{Acc.} & \textbf{MCC} & \textbf{Acc.} & \textbf{MCC} \\ \midrule
\multicolumn{3}{c}{\textbf{Encoder LMs}} \\ \midrule

ruBERT-base & 74.50 \tiny{$\pm$ 0.60} & 0.41 \tiny{$\pm$ 0.01} \\

ruBERT-large & 75.90 \tiny{$\pm$ 0.42} & 0.42 \tiny{$\pm$ 0.01} \\

ruRoBERTa-large & \underline{80.80} \tiny{$\pm$ 0.47} & \underline{0.54} \tiny{$\pm$ 0.01} \\

ruELECTRA-small & 61.74 \tiny{$\pm$ 1.09} & 0.20 \tiny{$\pm$ 0.02} \\

ruELECTRA-medium & 74.11 \tiny{$\pm$ 0.85} & 0.38 \tiny{$\pm$ 0.02} \\

ruELECTRA-large & 65.6 \tiny{$\pm$ 0.65} & 0.20 \tiny{$\pm$ 0.02} \\

mBERT & 67.47 \tiny{$\pm$ 1.33} & 0.19 \tiny{$\pm$ 0.01} \\ 

ruBERT-base (DP) & 72.57 \tiny{$\pm$ 1.92} & 0.35 \tiny{$\pm$ 0.12} \\

ruBERT-base-conv (DP) & 75.33 \tiny{$\pm$ 1.55} & 0.38 \tiny{$\pm$ 0.02} \\ 

RuLeanALBERT & 80.00 \tiny{$\pm$ 0.0} & 0.52 \tiny{$\pm$ 0.0} \\ 


XLM-R & 65.73 \tiny{$\pm$ 2.33} & 0.17 \tiny{$\pm$ 0.04} \\
RemBERT & 76.21 \tiny{$\pm$ 0.33} & 0.44 \tiny{$\pm$ 0.01} \\ 

\midrule \multicolumn{3}{c}{\textbf{Decoder LMs (PenLP)}} \\ \midrule
ruGPT-3-small & 53.89 \tiny{$\pm$ 0.0} & 0.25 \tiny{$\pm$ 0.0} \\

ruGPT-3-medium & 55.79 \tiny{$\pm$ 0.0} & 0.27 \tiny{$\pm$ 0.0} \\

ruGPT-3-large & 56.83 \tiny{$\pm$ 0.0} & 0.29 \tiny{$\pm$ 0.0} \\

mGPT-XL & 60.60 \tiny{$\pm$ 0.0} & 0.27 \tiny{$\pm$ 0.0} \\

\midrule

\multicolumn{3}{c}{\textbf{Encoder-decoder LMs}} \\ \midrule

ruT5-base & 71.26 \tiny{$\pm$ 1.31} & 0.27 \tiny{$\pm$ 0.03} \\

ruT5-large & 74.29 \tiny{$\pm$ 3.80} & 0.37 \tiny{$\pm$ 0.07} \\

FRED-T5-large & 75.83 \tiny{$\pm$ 0.0} & 0.40 \tiny{$\pm$ 0.0} \\

FRED-T5-XL & 77.37 \tiny{$\pm$ 0.0} & 0.46 \tiny{$\pm$ 0.0} \\ 

mT5-base & 64.64  \tiny{$\pm$ 0.0} & 0.15 \tiny{$\pm$ 0.0} \\ 

mT5-large & 63.85 \tiny{$\pm$ 0.0}  & 0.19 \tiny{$\pm$ 0.0}  \\ \midrule

Human & \textbf{84.08}  & \textbf{0.63} \\ \bottomrule
\end{tabular}}
\caption{Results on the RuCoLA test set. DP=DeepPavlov~\cite{burtsev-etal-2018-deeppavlov}. The best score is in bold, and the second best is underlined.}
\label{tab:rucola-results}
%\vspace{-2ex}
\end{table}
